Provenance-aware Discovery of Functional Dependencies on Integrated Views

The automatic discovery of functional dependencies(FDs) has been widely studied as one of the hardest problems in data profiling. Existing approaches have focused on making the FD computation efficient while inspecting single relations at a time. In this paper, for the first time we address the problem of inferring FDs for multiple relations as they occur in integrated views by solely using the functional dependencies of the base relations of the view itself. To this purpose, we leverage logical inference and selective mining and show that we can discover most of the exact FDs from the base relations and avoid the full computation of the FDs for the integrated view itself, while at the same time preserving the lineage of FDs of base relations. We propose algorithms to speedup the inferred FD discovery process and mine FDs on-the-fly only from necessary data partitions. We present InFine(INferred FunctIoNal dEpendency), an end-to-end solution to discover inferred FDs on integrated views by leveraging provenance information of base relations. Our experiments on a range of real-world and synthetic datasets demonstrate the benefits of our method over existing FD discovery methods that need to rerun the discovery process on the view from scratch and cannot exploit lineage information on the FDs. We show that InFine outperforms traditional methods necessitating the full integrated view computation by one to two order of magnitude in terms of runtime. It is also the most memory efficient method while preserving FD provenance information using mainly inference from base table with negligible execution time.

==> baseline_backup.tex <==


\section{Experiments}

\label{sec:experiments}

{\bf Evaluation Goal.} A fair comparison requires the preservation of FD provenance information. To do so, we compare our method which discovers FDs from a SPJ query specification and base tables against the straightforward approach that consists of discovering all the FDs from each base table, computing the query result, and discovering the FDs from the query result. The two main points we seek to validate are: (1) Does our approach enable us to discover FDs accurately (i.e., high precision) in an efficient manner and faster than the straightforward approach? (2) What is the impact of different data and SPJ query characteristics on \jedi performance? %

{\bf Setup.} We perform all experiments on a laptop Dell XPS machine with an Intel Core i7-7500U quad-core, 2.8 GHz, 16 GB RAM, powered by Windows 10 64-bit. %
Our algorithm implementation in Java use only one thread. Our code, scripts, data sets, and SPJ queries are available at \url{https://github.com/xxxx}. 



\begin{table}[t]
\centering
\small
\begin{tabular}{|c|l|r|r|}
\hline
{\bf DB} & {\bf Table}& {\bf (Att\# ; Tuple\#) }&{\bf FD\#}\\
\hline
\hline
 &{\bf Patients}& (7 ; 46.52k)& 11 \\
MIMIC3& {\bf Admissions}& (18 ; 58.976k)& 631\\
&{\bf Diagnoses\_icd}& (4 ; 651.047k)  & 2\\
&{\bf D\_icd\_Diagnoses}& (3 ; 14.710k)& 2\\
\hline
&{\bf active}& (2; 300)& 1\\
PTE&{\bf bond}&(4 ; 9.317k)& 3\\
&{\bf atm}& (5 ; 9.189k)& 5\\
&{\bf drug}& (1 ; 340)& 0\\
\hline
&{\bf atom}& (3; 12.333k)& 2\\
PTC&{\bf connected}&(3 ; 24.758k)& 3\\
&{\bf bond}& (3 ; 12.379k)& 2\\
&{\bf molecule}& (2 ; 343)& 1\\
\hline
&{\bf Supplier}& (7 ; 10k)& 34 \\
TPC-H&{\bf Customer}&(8 ; 150k)& 51\\
&{\bf Orders}& (9 ; 1.5M)& 53 \\
&{\bf LineItem}& (16 ; 6M)& 3946 \\
&{\bf Nation}& (4 ; 23)& 9 \\
&{\bf Region}& (3 ; 5)& 6 \\
&{\bf Part}& (7 ; 200k)& 99 \\
&{\bf Partsupp}& (5 ; 800k)&11 \\
\hline
\end{tabular}
\caption{Data characteristics.
}\label{exp:tables}
\end{table}


 
{\bf Data.}
We use  three  real-world  datasets  and  one  synthetic data set in our experiments: (1) the clinical database {\tt MIMIC-3}\footnote{\url{https://physionet.org/content/mimiciii/1.4/}} \cite{mimiciii}; 
 (2) PTE\footnote{\url{https://relational.fit.cvut.cz/dataset/PTE}}, a database for predictive toxicology evaluation, used to predict whether the compound is carcinogenic, and (3) PTC\footnote{\url{https://relational.fit.cvut.cz/dataset/PTC}}, the data set from the Predictive Toxicology Challenge that consists of more than three hundreds of organic molecules marked according to their carcinogenicity on male and female mice and rats; and (4) the TPC-H Benchmark\footnote{\url{http://www.tpc.org/tpch/}} with scale-factor 1. 
Data sets characteristics are given in Table \ref{exp:tables} and the characteristics of the queries in Table \ref{exp:spj}. 
All the datasets used  in the literature for benchmarking FD discovery methods consist of single tables.  Since we need to manipulate multiple tables with SPJ queries, we could not used them for our experiments and therefore, we propose our own benchmark. We adapted TPC-H queries by removing group-by and order-by statements and used the same constants specified in query validation sections of the documentation\footnote{\url{http://tpc.org/tpc_documents_current_versions/pdf/tpc-h_v3.0.0.pdf}}. 


{\bf Methods.} We compare \jedi algorithms applied to base tables only  %
against four state-of-the-art FD discovery methods: (1) TANE \cite{HKPT98,HKPT99},   (2) Fast\_FDs \cite{WGR01}, and (3) FUN \cite{NoCi01icdt}, and (4) HyFD \cite{HyFD}, using Java implementation of Metanome \cite{Papenbrock:2015} with command line. %
Data sets are stored in a Postgres DBMS. Join attributes are indexed with B-Tree and hash indexes. We averaged the results  over 10 runs for each query. %


\begin{table}[t]
\centering
\small
\begin{tabular}{|p{1cm}|p{4.8cm}|r|r|}
\hline
{\bf DB} & {\bf SPJ Query}&   {\bf Tup\#} & {\bf FD\#}\\
\hline
\hline
MIMIC3&patients $\bowtie$  admissions &58,976 & ???\\
&	diagnosesicd $\bowtie$  patients&58,798&12\\
&	dicddiagnoses $\bowtie$  diagnosesicd	&658,498&22\\
&	[diagnosesicd$\bowtie$patients]$\bowtie$ dicddiagnoses&	658,498&44\\
\hline
PTC	
&	atom $\bowtie$  molecule&	9,111&4\\
&connected $\bowtie$  bond&24,758&8\\
&	[connected $\bowtie$  bond] $\bowtie$  molecule	&18,312&12\\
&	connected $\bowtie_{id1}$ [atom $\bowtie$  molecule]&	18,312&12\\

\hline
PTE	&	atm $\bowtie$  drug&	9,189&5\\
&active $\bowtie$  drug&299&1\\
&	[bond $\bowtie$  drug] $\bowtie$  active&7,994&6\\

&	[atm $\bowtie$  bond $\bowtie$  atm] $\bowtie$  drug&	9,317&24\\
\hline
TPC-H%
& Q2$^*$(P $\bowtie$ PS $\bowtie$ S $\bowtie$ N $\bowtie$ R)  
& 	

21,696& 67\\
& Q3$^*$(C $\bowtie$ O $\bowtie$ L) 
&60,150&10 \\
& Q4$^*$(O $\bowtie$ L) 
&894,773&44 \\
& Q7$^*$(S $\bowtie$ L $\bowtie$ O $\bowtie$ C $\bowtie$ N1 $\bowtie$ N2)   &97,104&149,532 \\
& Q9$^*$(P $\bowtie$ PS $\bowtie$ S $\bowtie$ L $\bowtie$ O $\bowtie$ N)   &3,735,632&8 \\
& Q10$^*$(C $\bowtie$ O $\bowtie$ L $\bowtie$ N)  &2,683,532& 61\\
& Q11$^*$(P  $\bowtie$ S $\bowtie$ N)  
&284,160&104 \\
& Q14$^*$(L  $\bowtie$ P) 
&149,954& 52,417\\
\hline
\end{tabular}
\caption{SPJ queries considered in our experiments.
}\label{exp:spj}
\end{table}




{\bf Metrics.}  
 We examine precision, average runtime, and  maximal memory consumption for each query over 10 runs.  %
 Precision is defined as the fraction of correctly discovered FDs  by \jedi  from the base tables that are common with the FDs discovered from the SPJ query result by the straightforward method over the total number of discovered FDs. %
We compare execution times as follows: \jedi is applied to the base tables and receives their respective FDs as inputs, and we report its average execution time over 10 runs. The competing methods are applied to each SPJ query result and we report their average execution time over 10 runs to which we added the SPJ query execution time. 

We observed that the cardinalities and overlap of the join attribute values are rarely preserved through a join operation and this has a great impact on FD discovery depending on the join operator used. %
To quantify this phenomenon, we define the coverage as a metric computed as follows:
\begin{align*}
   Coverage(R\Diamond L) =
       \frac{1}{2}  \bigg( &Cov(R\Diamond L, L, X) + Cov(R\Diamond L, R, Y)\bigg)
    \\
    \text{with }Cov(Join, I, a) &= \frac{1} {|\pi_{a}(I) |} \sum\limits_{\forall v \in \pi_{a}(I)} 
                \frac{|\sigma_{a=v}(Join)) |}
                     {|\sigma_{a=v}(I) |}.
\end{align*}
  $X$ and $Y$ denote the join attributes of $\leftInst$ and $\rightInst$ base relations, respectively. $I$ is a considered instance and $a$ the considered join attribute. If $Coverage(R\Diamond L)=0$, no tuple from $L$ can be joined with tuples in $R$. For $Coverage(R\Diamond L)<1$, some tuples in $L$ (or $R$) may be missing from the join result, as it is the case for patients \#257 in {\small\texttt{PATIENT}} and \#247, \#248, and \#253 in {\small\texttt{ADMISSION}} that do not have their counterparts in the other table in our example. For $Coverage(R\Diamond L)=1$, there are as many tuples in both tables $L$ and $R$ as in the join result. For $Coverage(R\Diamond L)>1$, there are more tuples in the join result than in tables $L$ or $R$ as some tuples may be repeated through the join.%
 
 
 


\begin{figure}[!t]
	\centering
	\includegraphics[width=\linewidth]{figures/fig3-new.pdf}
	\caption{Average runtime of \jedi against FUN, TANE, FastFDs, and HyFD algorithms}\label{fig:jedi-time-comparison}
\end{figure} 
 \begin{figure*}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/fig4-new.pdf}
	\caption{Maximal memory consumption of \jedi against FUN, TANE, HyFD and FastFDs  algorithms}\label{fig:jedi-memory}
\end{figure*} 

\subsection{Efficiency and Effectiveness Evaluation}
In a first set of experiments, we evaluate the runtime and memory consumption of \jedi algorithms compared to the state-of-the-art FD discovery methods that follow the straightforward approach over 34 SPJ queries on the real-world and synthetic data sets with various coverage values.  The selected queries are representative in terms of coverage. Results for other queries are available as supplementary material on Github. %










\subsubsection{Runtime} 
Figure~\ref{fig:jedi-time-comparison} presents,  for each method, the average total runtime in seconds for FD discovery (including data loading). For the competing methods, we  added the average execution time of the SPJ query over the indexed data. Our method does not require the full SPJ query computation to discover FDs. Overall \jedi  is much faster than the traditional methods operating on the pre-computed full join results with one order of magnitude on average. %
However, for MIMIC3 and joins with higher coverage, \jedi  is not as competitive as HyFD applied to the full join result. This result actually motivated the design of a sampling-based method that can be more efficient when join coverage is high ($\log(Coverage)>1$) in large table sizes (i.e., when many tuples from one table are repeated in the join operation).  \jedi shows  better performances for low coverage joins PTE and PTC with a sampling size around 28\% in average to reach precision of 1. However, when both join coverage and table size increase, \jedi needs 63\% of the sample size on average to reach precision 1 as shown for MIMIC3 to compete with HyFD that operates over the precomputed full join. Also, the figure shows that both variants of \jedi are sensitive to the table ordering in the join operation, even more when the join size increases. %

\subsubsection{Memory Consumption} As shown in  Figure~\ref{fig:jedi-memory}, average maximal memory consumption of \jedi is the lowest for PTE and PTC data sets with low coverage. Memory consumption of \jedi  (when precision is 1) is between xxx\% and xx\% lower than xxx on average for PTE and PTC and, which makes it perform better than HyFD in certain cases. However, for MIMIC3 as the number of attributes and the coverage increase, HyFD generally outperforms the other methods with \jedi  has the second position.  %


 \begin{figure*}[t]
	\centering
		\includegraphics[width=.98\linewidth]{figures/time-rep6.pdf}
		
	\caption{Average runtime of \jedi with breakdown per algorithm %
	}
	\label{fig:jedi-time-repartition}
\end{figure*} 


\subsection{Evaluation}
In Figure~\ref{fig:jedi-time-repartition},  we report the average runtime breakdown of each algorithm 1, 2, and 3 in \jedi (in the horizontal histograms) and their respective percentages of discovered FDs (in the adjacent pie charts with the same color coding). Error bars represent the standard deviation of the average total runtime of the algorithms over ten runs.  The data distributions, cardinalities of the join attribute values, and the join coverage have very different characteristics across the data sets to illustrate the behavior of our algorithms on different join orderings and different coverage values for PTC and MIMIC3. We observe the same behavior in PTE which is not shown due to space limitation. %
Algorithm 1 manipulates different sets of upstaged AFDs per input table, as we can see with the 3-size joins in MIMIC3. The logical inference made by Algorithm 2 from Algorithm 1 output will lead to different resulting sets of inferred FDs. For MIMIC3, \jedi 1 alone retrieves 52\% of the true FDs on average. Algorithm 2 helps only for {\small\texttt{patients}} $\bowtie$ [{\small\texttt{diagnoseicd}} $\bowtie$ {\small\texttt{dicddiagnoses}}], the only case when the logical inference can be triggered from the FDs discovered by Algorithm 1.  

 The figure shows that different orderings in the tables participating in the join operations change not only the runtime but also the contribution of each algorithm in retrieving the true FDs. The reason is that various orderings of the input tables lead to different sets of potential upstaged AFDs and  trigger different logical inferences. Consequently, the remaining set of join FDs to discover (by Algorithm 3 or 4) will be different. Future work will be to find the optimal ordering of the input tables %
 and predict the cases where logical inference could prevail over selective mining to discover FDs more efficiently. %
 










\begin{table*}[t]
\centering
\scriptsize
\begin{tabular}{|p{1cm}|p{4.2cm}|r|r|r|r}
\hline
{\bf Data set} & {\bf SPJ Query}& {\bf Cov. } & Algo 1 FD\# & Algo 2 FD\# & Algo 3 FD\#\\
\hline
MIMIC-3&patients $\bowtie$  admissions&	1.13 & & &\\
&	diagnosesicd $\bowtie$  patients&	7.50& & &\\
&	dicddiagnoses $\bowtie$  diagnosesicd	&22.84& & &\\
&	[diagnosesicd$\bowtie$patients]$\bowtie$ dicddiagnoses&	22.84& & &\\
\hline
PTC	
&	atom $\bowtie$  molecule&	13.67& & &\\
&connected $\bowtie$  bond&	1.50&24,758 & &\\
&	[connected $\bowtie$  bond] $\bowtie$  molecule	&27.08& & &\\
&	connected $\bowtie_{id1}$ [atom $\bowtie$  molecule]&	27.08& & &\\

\hline
PTE	&	atm $\bowtie$  drug&	14.01& & &\\
&active $\bowtie$  drug&	0.94& & &\\
&	[bond $\bowtie$  drug] $\bowtie$  active&	13.83& & &\\

&	[atm $\bowtie$  bond $\bowtie$  atm] $\bowtie$  drug&	14.20& & &\\
\hline
TPC-H%
& Q2$^*$(P $\bowtie$ PS $\bowtie$ S $\bowtie$ N $\bowtie$ R)  
& 	

0.07& & &\\
& Q3$^*$(C $\bowtie$ O $\bowtie$ L) 
&0.44& & &\\
& Q4$^*$(O $\bowtie$ L) 
&& & &\\
& Q7$^*$(S $\bowtie$ L $\bowtie$ O $\bowtie$ C $\bowtie$ N1 $\bowtie$ N2)   && & &\\
& Q9$^*$(P $\bowtie$ PS $\bowtie$ S $\bowtie$ L $\bowtie$ O $\bowtie$ N)   && & &\\
& Q10$^*$(C $\bowtie$ O $\bowtie$ L $\bowtie$ N)  &9.84& & &\\
& Q11$^*$(P  $\bowtie$ S $\bowtie$ N)  
&& & &\\
& Q14$^*$(L  $\bowtie$ P) 
&0.39& & &\\
\hline
\end{tabular}
\caption{Repartition of FDs inferred nd discovered.
}\label{exp:spj}
\end{table*}







This shows the main advantage of our approach, reducing drastically the execution time of the join FD discovery.
Table \ref{tab:exp-jedi4}  completes the comparative study of the two variants of \jedi against the competing methods for the worst case scenarios when join coverage is high for large table size. Recall that \jedi  has shown the best performances over the state-of-the-art methods for PTE and PTC joins with relatively low join coverage and small table sizes (from 2 to 5 attributes and 300 to 24k tuples). So, we focus on MIMIC3 and TPC-H joins and report for each join: its coverage, the Join size ratio (expressed as  the sample size over the full join size, and as a percentage in parentheses, and the average runtime of \jedi  at precision 1, FUN, TANE, HyFD, and FastFDs. 

For MIMIC3, we observe that \jedi outperforms all the methods with at least one of the variants of the join ordering, otherwise HyFD applied to the full join result is slightly faster. This shows that the ordering of large tables is critical for size 3 and more joins but most importantly, high coverage impacts the sampling strategy. The reason is that many tuples from each input table are repeated through the join operation and the choice of more than one representative tuples jeopardizes the sampling result, in particular when it does not preserve the balance and distributions of the repeated tuples from the full join to the multiple micro-joins. 

For TPC-H, we observe the same phenomenon for the 3-size join  where the straightforward approach with HyFD is slighlty more efficient (or equal with TANE). We observe that the join size ratio to reach precision 1 is influenced by the coverage and also the number of distinct values for each attributes of the joined tables. For example, for the join {\small \texttt{part}}$\bowtie {\small \texttt{partsupp}}$, the average number of distinct values per attribute is 52,984 for {\small \texttt{part}}  and 223,971  for {\small \texttt{partsub}} which facilitates the sampling strategy in selecting violating tuples and reducing the space of candidates FDs. This can explain the relatively low ratio (22\%) despite high join  coverage.

These observations show that there is room for improvement  in the two following directions: (1) to find the optimal ordering of the tables to maximize the performance of FD discovery (in particular in Algorithm 1) and and (2) to improve the sampling strategy and better tune the sample size $n_b$ to maximize the number of violations and reduce the space of candidate join FDs.

==> sampling.tex <==
\subsubsection{Sampling-based Discovery of Join FDs}
As the computation of the join FDs by Algorithm~\ref{algo:MultiInst_CrossJoinFDs} can be expensive both in time and space, we propose Algorithm~\ref{algo:statisticalInferenceJoinFDs} which relies on selective sampling. To this extent, Algorithm~\ref{algo:statisticalInferenceJoinFDs} starts with the \texttt{micro\_join} subroutine that compute FDs from micro-joins only between the tuples from $L$ and $R$ that are selected by the \texttt{selective\_sampling} subroutine (lines \#6 and \#19--25).  The set of tuple ids to join is generated in the \texttt{generate\_ids\_set} subroutine  (lines \#23-24, \#26-38). It builds a tree where the depth levels correspond to the order of the attributes  with the fewest number of distinct values as the first level and $n_v$ the last level to consider (line \#29); the nodes correspond to  distinct values per attribute (i.e., level) (line \#33). Then, if an attribute value corresponds to a unique tuple for a level less than $n_v$, the tuple id is selected as the representative tuple of a branch to be considered for the micro-join; if multiple tuples share the same value, $n_b$ tuples will be selected.
Then, for each sample, the instances are joined (line\#~\ref{line:joinPair}) and the FDs over the resulting instance are computed and added to  $\mathcal{E}_{out}$, the set of all computed FDs  (lines\#~\ref{line:computeFDsPairs} and \ref{line:addNewFDsPairs}).
Finally, subroutine \texttt{computeLvLFDs} (line\#~\ref{line:callPartition}) extracts from the set $\mathcal{E}_{out}$ the FDs that are valid in every sample. An FD $d$ can be considered as valid in a set of FD $\fdSet$ if either (1) there exists a logically equivalent FD in $\fdSet$ or (2) there exists an FD logically implying $d$ in $\fdSet$. However, we cannot guarantee that an FD discovered from samples is exact in the joined instance without the full exploration. Indeed, %
for a given FD $d$, in the worst case, %
 the projection of $\leftInst\bowtie\rightInst$ over the attributes in $d$  needs to be explored to check the non-existence of a pair of tuples violating $d$. We refer to \cite{davies1994np} for a formal proof of the NP-completeness of finding minimal FDs.
\input{algorithms/algo3bis}






Algorithm 4 operates on micro-joins computed by {\small\texttt{micro\_join}} subroutine with complexity $|P_i| * ( O(|L_i| \cdot |R_i| ) +  O( |\mathcal{E}_{\mathcal{D}}|)$ with $|P_i|$ the number of tuples in the micro-join $i$, $|L_i|$ and $|R_i|$ the number of tuples in $L$ and $R$ participating to the micro-join, and  
$\mathcal{E}_{\mathcal{D}}$,  the set of consistent FDs discovered from multiple micro-joins FD sets. The complexity of selective sampling is $ O( |L| + |R| )  + O( n_v * k_{max} )$, with $k_{max}$, the maximum number of attributes in $L$ or $R$. 


\subsubsection{Completeness and Correctness of \jedi with sampling}
\jedi with sampling uses Algorithm 1 and 2 with the same completeness and correctness guarantees exposed previously for \jedi with selective mining.

The correctness of Algorithm~\ref{algo:statisticalInferenceJoinFDs}  cannot be guaranteed as there is a probability of not sampling a pair of counter-example tuples for a given AFD, and thus to confound the AFD with an exact FDs in the join results. Due to the NP-completeness of the minimal FD mining problem\cite{davies1994np}, every pair of tuples must be checked in order to find a possible counter-example, thus to guarantee that the discovered FDs from samples are exact FDs. We would like to note that developing a framework to guarantee the accuracy of the sampling-based FD discovery approach is a  challenging problem and a focus of our future research.


 Algorithm~4  uses Algorithm 3 over samples, the retrieved FDs are minimal exact FDs holding on the samples. If there exists a minimal FDs $A\to b$ in a sample, an FD $A^\prime \to b$ such that $A^\prime \subset A$ cannot become a minimal FD in the full instance. Therefore, the FDs retrieves in from the samples imply the set of FDs over the full joined instance.




\subsection{Evaluation of \jedi with Sampling }
In this last set of experiments, we evaluate \jedi 1,2,4 and show that it outperforms \jedi\_SM and other competing methods in terms of runtime for precision equals to 1, in particular for the worst case scenarios when coverage is high. First, we investigate the effect of the sample size on the precision of \jedi Algorithms 1,2, and 4. 
\begin{wrapfigure}{l}{0.25\textwidth}
	\centering
	\includegraphics[width=\linewidth]{figures/sample-size.pdf}
	\caption{Effect of sampling size on \jedi\_SB precision for  {\small\texttt{PATIENT}\_{{\small 1K}}} $\bowtie$ {\small\texttt{ADMISSION}\_{{\small 1K}}}  }\label{fig:sample-size}
\end{wrapfigure}
\noindent Figure \ref{fig:sample-size} shows precision of selective sampling with \jedi 1,2,4 compared to \jedi 1,2 followed by random sampling (averaged over 10 runs) for the inner join between 1,000 tuples of  {\small\texttt{PATIENT}}  and 1,000 tuples of {\small\texttt{ADMISSION}} with high \mbox{coverage (>1)} (cf. Figure \ref{fig:inner}(a)).  For this experiment, we used $n_b=1$ as input parameter for selective sampling to pick only one tuple as the representative tuple of a branch and we vary $n_v$ from 0 to $| atts({\small\texttt{PATIENT}}\bowtie{\small\texttt{ADMISSION}})|$ to exclude the attributes with the highest number of  distinct values. 
\jedi 1,2,4 reaches precision (and recall) of 1 when the size of the selected sample is 62.3\% of the table input size. Interestingly, even for a sample of size of 10\% with tuples selected by Algorithm 4, we can see an improvement of +0.153 over \jedi 1 and 2 precision. 


